Unveiling the Latent Space Geometry of Push-Forward Generative Models

Many deep generative models are defined as a push-forward of a Gaussian measure by a continuous generator, such as Generative Adversarial Networks (GANs) or Variational Auto-Encoders (VAEs). This work explores the latent space of such deep generative models. A key issue with these models is their tendency to output samples outside of the support of the target distribution when learning disconnected distributions. We investigate the relationship between the performance of these models and the geometry of their latent space. Building on recent developments in geometric measure theory, we prove a sufficient condition for optimality in the case where the dimension of the latent space is larger than the number of modes. Through experiments on GANs, we demonstrate the validity of our theoretical results and gain new insights into the latent space geometry of these models. Additionally, we propose a truncation method that enforces a simplicial cluster structure in the latent space and improves the performance of GANs.

==> dump.tex <==
\begin{itemize}
    \item EN COURS Generalize theorems to continuous distributions?
    \item DONE (nope) GANs with simplicial latent are the ONLY minimizers: wait for answers 
    \item DONE Remove theorem density/coverage and introduce more Improved/PR
    \item Impact of over-parametrization (width of generator) on convergence EN COURS
    \item EN COURS Vary number modes (check bounds $\sqrt{\log m}$): synthetic gaussians. On MNIST/CIFAR: 2 to 10 modes X different latent dim (5,10,30?). 
    \item TODO Intro according to reviewer remark: "Given the key idea from the soap bubble result I would talk about this result and why it is applicable to GANs generating disconnected manifolds, rather than starting with GANs and their measures of precision first. The idea is that in the optimal case the classes should be well separated with limited points on the boundary between classes (in the latent space). How this is quantified currently is then naturally motivated, and is just codification of that natural intuition."
    \item TODO: recheck reviews and derive according improvements for the paper.
    \item TODO: more discussions on the theoretical part: do assumptions correspond to the practice?, impact of theorems, etc. 
    \item TODO: Distance between barycenter of classes: is it equidistant? Try with normalization. 
    \item TODO: classification with nearest normalized barycenter. 
    \item TODO: our metrics with a SOTA GAN, e.g. TransGAN on CIFAR10
    \item TODO: try with more modes to observe $\sqrt{\log (m)}$ (>100?). Estimate L on the borders to get the rate.  
    \item TODO: new fig for linear interpolatio with TransGAN
    
    
\end{itemize}




CIFAR-2 & 5 & 80.0 $\pm$ 0.5 & 269.9 $\pm$ 34.1  & 65.5 $\pm$ 0.8  & 77.5 $\pm$ 1.9  & 54.2 $\pm$ 1.8  & 68.2 $\pm$ 2.1  \\
& 10 &  86.7 $\pm$ 0.5  & 254.3 $\pm$ 44.2  & 70.6 $\pm$ 0.6  & 77.5 $\pm$ 1.6  & 64.5 $\pm$ 1.4  & 74.8 $\pm$ 2.6 \\
 & 30 & 85.9 $\pm$ 0.2 & 189.7 $\pm$ 56.9  & 74.0 $\pm$ 0.8  & 76.6 $\pm$ 1.6  & 71.5 $\pm$ 2.0  & 78.0 $\pm$ 1.8  \\ 
 & 64 & 86.6 $\pm$ 0.3 & 205.4 $\pm$ 45.9  & 73.9 $\pm$ 0.8  & 77.0 $\pm$ 1.6  & 71.5 $\pm$ 1.6  & 78.2 $\pm$ 1.9 \\\hline 
 CIFAR-4 & 5 & 50.3 $\pm$ 0.5 & 42.7 $\pm$ 0.7 & 86.4 $\pm$ 0.3 & 30.1 $\pm$ 0.6 & 60.2 $\pm$ 0.6  \\ 
 & 10 &  75.3 $\pm$ 0.4 & 87.3 $\pm$ 4.1 & 69.6 $\pm$ 0.6 & 79.9 $\pm$ 0.3 & 65.6 $\pm$ 1.5 & 82.8 $\pm$ 0.5 \\ 
 & 30 & \\ 
 & 64 & 77.9 $\pm$ 0.4 & 109.5 $\pm$ 17.3  & 72.8 $\pm$ 0.5  & 78.6 $\pm$ 1.0  & 72.2 $\pm$ 1.1  & 82.9 $\pm$ 0.9 \\   \hline
  CIFAR-6 & 5 & 38.4 $\pm$ 0.5 & 187.9 $\pm$ 16.6  & 65.1 $\pm$ 0.5  & 80.4 $\pm$ 0.4  & 53.8 $\pm$ 1.0  & 73.9 $\pm$ 1.1 \\ 
 & 10 & 67.9 $\pm$ 0.3 & 121.5 $\pm$ 14.0  & 72.6 $\pm$ 0.4  & 79.8 $\pm$ 0.9  & 69.4 $\pm$ 1.2  & 81.7 $\pm$ 0.9 \\ 
 & 30 & 73.3 $\pm$ 0.4 & 89.9 $\pm$ 10.4  & 75.5 $\pm$ 0.5  & 79.3 $\pm$ 0.6  & 77.7 $\pm$ 1.3  & 85.4 $\pm$ 0.5 \\ & 64 & 72.4 $\pm$ 0.5  & 77.6 $\pm$ 12.2  & 76.2 $\pm$ 0.8  & 78.8 $\pm$ 1.8  & 79.2 $\pm$ 3.3  & 85.5 $\pm$ 1.0  \\ \hline
 CIFAR-8 & 5 & 37.1 $\pm$ 0.5 & 191.8 $\pm$ 9.9  & 64.6 $\pm$ 0.5  & 81.6 $\pm$ 0.6  & 52.9 $\pm$ 1.0  & 73.9 $\pm$ 1.0 \\ 
 & 10 & 59.6 $\pm$ 0.3 & 120.8 $\pm$ 11.7  & 70.7 $\pm$ 0.5  & 82.1 $\pm$ 0.4  & 65.0 $\pm$ 1.1  & 81.3 $\pm$ 1.1  \\
 & 30 & 67.7 $\pm$ 0.4 & 97.0 $\pm$ 9.6 & 74.3 $\pm$ 0.4  & 81.4 $\pm$ 0.6  & 73.6 $\pm$ 1.0  & 85.0 $\pm$ 0.8  \\ 
  & 64 &  67.1 $\pm$ 0.6 & 90.3 $\pm$ 13.6  & 74.6 $\pm$ 0.6  & 81.0 $\pm$ 1.2  & 74.4 $\pm$ 2.2  & 85.6 $\pm$ 1.3 \\ \hline
  
  
  
  
  
  
  OLD FULL RESULTS TABLE
  
  \begin{table}[H]
\begin{tabular}{l|c|c|c|c|c|c|c}
Dataset & L. Dim.  & Acc. & FD & Prec. & Rec. & Dens. & Cov. \\ \hline 
MNIST & 2 & 44.3 $\pm$ 2.5 & 112.3 $\pm$ 22.6 & 2.9 $\pm$ 1.0 & 89.1 $\pm$ 2.0 & 0.9 $\pm$ 0.3 & 2.1 $\pm$ 0.5 \\ 
& 4 & 59.4 $\pm$ 0.7 & 36.4 $\pm$ 9.3 & 75.7 $\pm$ 1.8 & 91.5 $\pm$ 0.5 & 47.9 $\pm$ 2.2 & 66.0 $\pm$ 2.0 \\
& 6 & 83.9 $\pm$ 0.4 & 15.4 $\pm$ 3.0 & 90.0 $\pm$ 0.7 & 92.4 $\pm$ 0.7 & 76.3 $\pm$ 2.0 & 85.8 $\pm$ 0.4 \\
 & 8 & 84.7 $\pm$ 0.4 & 18.2 $\pm$ 3.4 & 91.1 $\pm$ 0.7 & 92.3 $\pm$ 0.5 & 81.3 $\pm$ 2.2 & 87.1 $\pm$ 0.8 \\ 
  & 10 & 86.7 $\pm$ 0.4 & 10.7 $\pm$ 2.6 & 93.3 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 89.0 $\pm$ 2.2 & 89.8 $\pm$ 0.7 \\
  & 12 & 87.4 $\pm$ 0.4 & 7.2 $\pm$ 1.6 & 94.6 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 94.3 $\pm$ 2.0 & 91.8 $\pm$ 0.7 \\
  & 16 & 86.9 $\pm$ 0.4 & 11.0 $\pm$ 1.0 & 93.8 $\pm$ 0.3 & 91.8 $\pm$ 0.6 & 92.2 $\pm$ 0.9 & 90.7 $\pm$ 0.5 \\
  & 32 & 90.3 $\pm$ 0.4 & 10.4 $\pm$ 1.6 & 93.6 $\pm$ 0.3 & 91.6 $\pm$ 0.7 & 91.8 $\pm$ 1.7 & 90.3 $\pm$ 0.6 \\
  & 64 & 90.4 $\pm$ 0.3 & 13.3 $\pm$ 2.6 & 93.2 $\pm$ 0.4 & 92.3 $\pm$ 0.5 & 90.1 $\pm$ 2.0 & 90.2 $\pm$ 0.8 \\
  & 128 & 87.0 $\pm$ 0.4 &  11.0 $\pm$ 2.3 & 93.6 $\pm$ 0.3 & 91.8 $\pm$ 0.4 & 91.6 $\pm$ 1.5 & 90.4 $\pm$ 0.7 \\ \hline 
CIFAR-10 & 2 & 19.1 $\pm$ 1.1 & 408.3 $\pm$ 23.3 & 6.4 $\pm$ 0.9 & 79.5 $\pm$ 1.3 & 1.8 $\pm$ 0.3 & 3.9 $\pm$ 0.4 \\
& 4 & 27.4 $\pm$ 1.0 & 298.6 $\pm$ 38.1 & 59.2 $\pm$ 0.8 & 78.9 $\pm$ 0.8 & 42.9 $\pm$ 0.6 & 65.9 $\pm$ 0.7 \\
& 6 & 42.7 $\pm$ 0.6 & 142.6 $\pm$ 5.4 & 69.4 $\pm$ 0.6 & 76.6 $\pm$ 0.5 & 60.3 $\pm$ 1.1 & 76.3 $\pm$ 0.8\\
& 8 & 44.6 $\pm$ 0.6 & 174.7 $\pm$ 9.6 & 69.7 $\pm$ 0.7 & 79.6 $\pm$ 0.5 & 61.0 $\pm$ 1.4 & 77.8 $\pm$ 1.0\\
& 10 & 53.7 $\pm$ 0.4 & 134.7 $\pm$ 7.4 & 72.7 $\pm$ 0.6 & 76.6 $\pm$ 0.6 & 67.6 $\pm$ 1.3 & 80.4 $\pm$ 1.0 \\
& 12 & 58.2 $\pm$ 0.3 & 131.8 $\pm$ 8.5 & 74.0 $\pm$ 0.5 & 76.1 $\pm$ 0.6 & 71.3 $\pm$ 1.6 & 82.0 $\pm$ 1.1\\
& 14 & 60.1 $\pm$ 0.4 & 115.5 $\pm$ 12.7 & 74.0 $\pm$ 0.5 & 77.7 $\pm$ 0.8 & 72.4 $\pm$ 1.4 & 82.8 $\pm$ 0.9 \\
& 16 & 60.7 $\pm$ 0.4 & 145.9 $\pm$ 8.9 & 73.2 $\pm$ 0.7 & 78.5 $\pm$ 0.7 & 66.9 $\pm$ 1.3 & 79.6 $\pm$ 0.7\\
& 32 & 63.5 $\pm$ 0.2 & 126.5 $\pm$ 5.9 & 74.5 $\pm$ 0.5 & 79.1 $\pm$ 0.4 & 70.9 $\pm$ 1.5  & 82.0 $\pm$ 0.9 \\
& 64 & 64.0 $\pm$ 0.3 & 124.6 $\pm$ 4.5 & 74.0 $\pm$ 0.6 & 79.2 $\pm$ 0.3 & 71.2 $\pm$ 1.8 & 82.7 $\pm$ 1.0 \\ 
& 128 & 63.6 $\pm$ 0.4 & 132.6 $\pm$ 7.8 & 73.8 $\pm$ 0.5 & 79.2 $\pm$ 0.6 & 69.7 $\pm$ 1.2 & 82.1 $\pm$ 0.6 \\ \hline
 CIFAR-100 & 2 & 10.7 $\pm$ 1.4 & 2826.7 $\pm$ 837.3 & 1.4 $\pm$ 0.2 & 70.2 $\pm$ 1.1 & 0.3 $\pm$ 0.1 & 0.7 $\pm$ 0.1 \\ 
 & 8 & 15.2 $\pm$ 0.2 & 1112.3 $\pm$ 56.9 & 59.5 $\pm$ 0.8 & 62.8 $\pm$ 0.6 & 49.8 $\pm$ 1.6 & 70.5 $\pm$ 1.1\\
& 16 & 21.8 $\pm$ 0.3 & 1270.9 $\pm$ 89.7& 63.6 $\pm$ 1.3 & 61.3 $\pm$ 0.8 & 57.2 $\pm$ 2.8 & 73.9 $\pm$ 1.2 \\
& 32 & 23.9 $\pm$ 0.4 & 1068.0 $\pm$ 91.5 & 65.3 $\pm$ 0.4 & 62.1 $\pm$ 0.6 & 60.6 $\pm$ 1.1 & 77.4 $\pm$ 0.6 \\ 
& 64 & 25.1 $\pm$ 0.4 & 822.2 $\pm$ 50.5 & 66.5 $\pm$ 0.6 & 61.5 $\pm$ 0.8 & 64.0 $\pm$ 1.4 & 78.5 $\pm$ 0.8 \\
& 128 & 23.5 $\pm$ 0.3 & 963.0 $\pm$ 74.2 & 65.2 $\pm$ 0.7 & 62.2 $\pm$ 1.0 & 61.7 $\pm$ 1.6 & 77.4 $\pm$ 0.8 \\ 
& 256 & 21.2 $\pm$ 0.3 & 1086.6 $\pm$ 78.0 & 66.0 $\pm$ 0.5 & 60.2 $\pm$ 0.8 & 63.9 $\pm$ 1.2 & 78.1 $\pm$ 0.7 \\ 
& 512 & 20.6 $\pm$ 0.4 & 1128.7 $\pm$ 95.3 & 66.8 $\pm$ 0.6 & 61.1 $\pm$ 0.6 & 63.0 $\pm$ 1.2 & 77.6 $\pm$ 0.8 \\ \hline
CIFAR-3 & 2 & 44.8 $\pm$ 2.0 & 473.9 $\pm$ 55.0 & 5.3 $\pm$ 0.5 & 69.9 $\pm$ 2.1 & 1.5 $\pm$ 0.2 & 2.7 $\pm$ 0.4 \\
& 6 & 72.4 $\pm$ 0.4 & 169.2 $\pm$ 13.1 & 73.4 $\pm$ 0.8 & 69.7 $\pm$ 1.5 & 65.6 $\pm$ 1.5 & 72.7 $\pm$ 1.3 \\
& 8 & 78.4 $\pm$ 0.5 & 144.6 $\pm$ 8.2 & 74.9 $\pm$ 0.5 & 72.5 $\pm$ 1.4 & 71.0 $\pm$ 1.6 & 75.8 $\pm$ 1.7 \\ 
& 12 & 80.6 $\pm$ 0.4 & 135.2 $\pm$ 6.4 & 77.5 $\pm$ 0.5 & 71.2 $\pm$ 1.3 & 76.5 $\pm$ 1.1 & 78.3 $\pm$ 1.7 \\
& 16 & 80.9 $\pm$ 0.3 & 113.3 $\pm$ 9.0 & 78.7 $\pm$ 0.5 & 71.8 $\pm$ 1.5 & 80.7 $\pm$ 1.4 & 80.4 $\pm$ 1.4 \\ 
& 128 & 80.6 $\pm$ 0.1 & 115.3 $\pm$ 8.4 & 80.5 $\pm$ 0.7 & 70.4 $\pm$ 1.7 & 87.1 $\pm$ 2.1 & 82.7 $\pm$ 1.3 \\ \hline
Synthetic CIFAR-10 & 2 & 22.8 $\pm$ 2.2 & 234.6 $\pm$ 12.1 & 7.3 $\pm$ 1.3 & 71.7 $\pm$ 1.1 & 2.2 $\pm$ 0.4 & 4.6 $\pm$ 0.8 \\
& 4 & 33.8 $\pm$ 0.8 & 143.2 $\pm$ 15.0 & 60.3 $\pm$ 0.8 & 72.5 $\pm$ 0.8 & 44.4 $\pm$ 1.3 & 68.9 $\pm$ 1.2 \\ 
& 8 & 47.0 $\pm$ 0.6 & 85.5 $\pm$ 4.7 & 70.2 $\pm$ 0.3 & 72.5 $\pm$ 0.9 & 64.6 $\pm$ 0.6 & 83.2 $\pm$ 0.6 \\ 
& 10 & 52.6 $\pm$ 0.3 & 87.6 $\pm$ 5.4 & 70.4 $\pm$ 0.6 & 73.1 $\pm$ 0.7 & 66.2 $\pm$ 1.8 & 84.3 $\pm$ 0.7 \\
& 12 & 55.3 $\pm$ 0.4 & 84.3 $\pm$ 4.9 & 70.0 $\pm$ 0.5 & 73.5 $\pm$ 0.6 & 64.8 $\pm$ 1.2 & 83.6 $\pm$ 0.6 \\ 
& 16 & 59.1 $\pm$ 0.4 & 76.4 $\pm$ 6.1 & 71.6 $\pm$ 0.6 & 72.9 $\pm$ 1.2 & 68.7 $\pm$ 1.8 & 85.1 $\pm$ 0.4 \\
& 32 & 52.8 $\pm$ 0.2 & 73.4 $\pm$ 6.3 & 72.6 $\pm$ 0.5 & 72.2 $\pm$ 0.7 & 69.5 $\pm$ 1.4 & 85.7 $\pm$ 0.5 \\ 
& 128 &  58.7 $\pm$ 0.3 & 88.3 $\pm$ 6.2 & 70.1 $\pm$ 0.6 & 73.3 $\pm$ 0.6 & 66.3 $\pm$ 1.4 & 84.2 $\pm$ 0.8 \\ 
 \\
 \end{tabular}
\caption{Performance of GANs when varying latent space dimension. Confidence intervals are computed on 10 checkpoints of the same training. See main paper for curves of precision and FID with regard to the latent space dimension.\label{appendix:full_results} }
\end{table}
  
  
  

==> results_simplicial_rejection.tex <==






==> table_full_results_simplicial.tex <==
\begin{table*}
\tiny
\begin{tabular}{l|c|c|c|c|c|c|c|c}
Dataset   &  FD & Prec. & Dens. & Cov. & FID & Prec & Dens. & Cov.  \\ 
& & & & & (Incep.) & (Incep.) & (Incep.) & (Incep.) \\ \hline
CIFAR-10  & 75.8 $\pm$ 8.6  & 75.6 $\pm$ 0.4  &  76.9 $\pm$ 1.3 & {87.5 $\pm$ 0.8} & 16.5 $\pm$ 0.5 & 66.4 $\pm$ 0.5 %66.2 $\pm$ 1.0 
& 72.3 $\pm$ 1.5 &  75.6 $\pm$ 1.0 \\ 
Simplicial, n=10 (0.13,0.13) & & & & & 16.2 $\pm$ 0.4 
& 65.9 $\pm$ 0.6 
%66.2 $\pm$ 0.6 
& 70.2 $\pm$ 2.1 
& 75.4 $\pm$ 1.2  \\
Simplicial, n=10 (0.12,0.12) & & & & & 15.7 $\pm$ 0.3 
& 66.4 $\pm$ 0.6 
%65.9 $\pm$ 0.6 
& 71.5 $\pm$ 1.2 
& 75.9 $\pm$ 0.8 \\
Simplicial, n=10 (0.12,0.13) & & & & & 14.7 $\pm$ 0.3 
& 65.6 $\pm$ 0.4 
%66.6 $\pm$ 0.5 
& 68.9 $\pm$ 1.3 
& 75.8 $\pm$ 0.4 \\
  & \\\hline 
TransGAN & 340.1 & 79.9 &  91.4 & 90.0 & 8.9 $\pm$ 0.1  & 72.8 $\pm$ 0.8 & 79.3 $\pm$ 0.9  & 79.3 $\pm$ 1.2   \\ \hline 
TransGAN + 90\% JB-truncation & & & & & 8.7 $\pm$ 0.1 & 73.0 $\pm$ 0.6 & 83.5 $\pm$ 1.7 & 80.0 $\pm$ 1.6 \\
TransGAN + 80\% JB-truncation & & & & & 8.8 $\pm$ 0.1 & 73.3 $\pm$ 0.8 % & 61.2 $\pm$ 1.0
& 85.7 $\pm$ 2.8 & 81.1 $\pm$ 0.6 \\\hline
TransGAN + DeliGAN & & & & & 9.8 $\pm$ 0.1 
 & 74.6 $\pm$ 0.8  & 93.2 $\pm$ 2.8  & 80.0 $\pm$ 0.6 \\ \hline
 TransGAN + DeliGAN 100 & & & & & \\ 
 TransGAN + DeliGAN simp 10 & & & & & 8.8 $\pm$ 0.1 
& 73.7 $\pm$ 0.7 
%61.5 $\pm$ 2.1 
& 83.7 $\pm$ 2.3 
& 81.0 $\pm$ 0.9 \\
 TransGAN + DeliGAN simp 100 & & & & \\ \hline 
TransGAN + linear frontiers (tr=0.23,te=0.23) & & & & & 9.2 $\pm$ 0.1 & 73.1 $\pm$ 1.1 & 78.1 $\pm$ 2.7 & 79.4 $\pm$ 0.9 \\
(tr=0.23,te=0.29) & & & & & 9.2 $\pm$ 0.1 & 73.7 $\pm$ 0.8 & 83.4 $\pm$ 3.3 & 79.8 $\pm$ 0.5 \\ 
 (tr=0.23,te=0.31) & & & & & 9.3 $\pm$ 0.1 & 74.0 $\pm$ 0.5 & 86.1 $\pm$ 1.8 & 81.3 $\pm$ 0.7 \\
 (0.23,0.4) & & & & & 9.8 $\pm$ 0.1 
& 75.1 $\pm$ 0.8 
%59.8 $\pm$ 1.2 
& 89.5 $\pm$ 1.6 
& 80.5 $\pm$ 1.2 \\ \hline
TransGAN + non-linear frontiers (0.16,0.16) & & & & & 8.9 $\pm$ 0.1 & 73.9 $\pm$ 1.0 & 82.9 $\pm$ 2.3 & 80.6 $\pm$ 0.5 \\ 
(0.16,0.19) & & & & & 8.9 $\pm$ 0.1 & 74.1 $\pm$ 0.7 & 85.7 $\pm$ 3.5 & 81.2 $\pm$ 0.8 \\ 
(0.16,0.22) & & & & & 9.2 $\pm$ 0.1 & 75.8 $\pm$ 1.0 & 93.0 $\pm$ 4.2 & 81.0 $\pm$ 0.5 \\ 
(0.16,0.25) & & & & & 10.2 $\pm$ 0.1 & 77.4 $\pm$ 1.4 & 99.8 $\pm$ 3.6 & 80.9 $\pm$ 0.9 \\ \hline
TransGAN n=5  & \\
train threshold=0.25, test=0.25 & 478.9 $\pm$ 6.6 & 79.7 $\pm$ 0.4  & 90.9 $\pm$ 0.6  & 86.0 $\pm$ 0.4 & 8.8 $\pm$ 0.0  & 74.1 $\pm$ 0.9  & 85.9 $\pm$ 2.5  & 81.1 $\pm$ 0.3  \\ 
train threshold=0.25,test=0.255 & 586.6 $\pm$ 4.1 & 79.9 $\pm$ 0.3 & 91.7 $\pm$ 1.6 & 83.6 $\pm$ 0.6 & 8.8 $\pm$ 0.0 & 74.0 $\pm$ 1.0  & 88.4 $\pm$ 1.6  & 81.5 $\pm$ 0.5  \\ 
train threshold=0.24, test=0.24 & & & & & 9.5 $\pm$ 0.0 & 73.5 $\pm$ 0.3 & 82.5 $\pm$ 1.9 & 79.2 $\pm$ 0.9 \\ 
train threshold=0.24,test=0.25  & & & & & 9.5 $\pm$ 0.0 &  74.5 $\pm$ 0.3 & 89.3 $\pm$ 1.5 & 81.8 $\pm$ 0.3\\ 
tr thr=0.24,test=0.255 & & & & & 9.6 $\pm$ 0.1  & 74.6 $\pm$ 0.4  & 94.8 $\pm$ 1.9 & 81.4 $\pm$ 0.2 \\ \hline 
TransGAN n=10 & \\ 
train threshold=0.135,test=0.135 & & & & & 9.0 $\pm$ 0.0  & 72.9 $\pm$ 0.5  & 82.7 $\pm$ 1.9  & 80.4 $\pm$ 0.7 \\ 
0.135,0.138 & & & & & 8.9 $\pm$ 0.1 & 74.6 $\pm$ 0.7  & 85.9 $\pm$ 2.3 & 81.0 $\pm$ 0.5 \\
0.135,0.14 & & & & & 9.0 $\pm$ 0.1  & 74.2 $\pm$ 1.5  & 88.5 $\pm$ 3.1  & 81.3 $\pm$ 1.4 \\
0.135,0.142 & & & & & 9.1 $\pm$ 0.1 & 75.1 $\pm$ 0.7  & 93.3 $\pm$ 2.5  & 81.5 $\pm$ 0.8 \\ 
0.135,0.143 & & & & & 9.2 $\pm$ 0.1 & 74.9 $\pm$ 1.0  & 96.4 $\pm$ 2.2  & 82.6 $\pm$ 0.4 \\ 
0.135,0.144 & & & & & 9.3 $\pm$ 0.0 & 74.9 $\pm$ 0.8 & 95.0 $\pm$ 1.0 & 82.1 $\pm$ 0.5 \\
0.135,0.1445 & & & & & 9.3 $\pm$ 0.0 & 75.3 $\pm$ 0.6 & 98.6 $\pm$ 1.3 & 82.9 $\pm$ 0.5 \\\hline 
TransGAN n=10, loss=0.1 & \\ 
train threshold=0.135,test=0.135 & & & & & 8.5 $\pm$ 0.1  & 74.2 $\pm$ 0.9 & 84.7 $\pm$ 2.3 & 81.8 $\pm$ 0.9 \\ 
0.135,0.14 & & & & & 8.5 $\pm$ 0.0 & 74.0 $\pm$ 0.4 & 86.1 $\pm$ 1.3 & 82.3 $\pm$ 0.6\\
0.135,0.142 & & & & & 8.5 $\pm$ 0.0 & 74.5 $\pm$ 0.5 & 87.0 $\pm$ 0.7 & 82.8 $\pm$ 0.8 \\ 
0.135,0.143 & & & & & 8.5 $\pm$ 0.1 & 73.8 $\pm$ 0.6 & 84.3 $\pm$ 1.4 & 82.1 $\pm$ 0.7 \\ \hline 
train threshold=0.13,test=0.13 & & & & & 9.3 $\pm$ 0.1 & 73.3 $\pm$ 0.5 & 84.7 $\pm$ 1.9  & 80.9 $\pm$ 0.6 \\ 
train threshold=0.13,test=0.135 & & & & &  9.3 $\pm$ 0.1  & 73.5 $\pm$ 0.7  & 87.2 $\pm$ 3.5  & 80.6 $\pm$ 1.0 \\

train threshold=0.12,test=0.12 & & & & & 9.8 $\pm$ 0.1 & 73.8 $\pm$ 0.9 & 84.0 $\pm$ 2.8 & 79.4 $\pm$ 0.3 \\ 
train threshold=0.12,test=0.13 & & & & & 10.0 $\pm$ 0.1 & 74.2 $\pm$ 0.4 & 84.3 $\pm$ 2.2 & 78.9 $\pm$ 0.3 \\ 
train threshold=0.12,test=0.14 & & & & & 10.5 $\pm$ 0.1 & 74.7 $\pm$ 0.4 & 85.1  $\pm$ 2.2 & 78.6 $\pm$ 0.3 \\ 

\hline
CIFAR-100 & \\ \hline 
TransGAN& & & & & 15.2 $\pm$ 0.1 & 64.2 $\pm$ 0.5 & 53.4 $\pm$ 1.3  & 66.0 $\pm$ 1.1\\ \hline
TransGAN Deligan 10 & & & & & 15.9 
& 63.5 %62.2 $\pm$ 0.7 
& 52.6 & 64.4\\
TransGAN DeliGAN 100 & & & & & 15.3 $\pm$ 0.1 
& 64.2 $\pm$ 0.5 
%61.9 $\pm$ 0.9 
& 52.6 $\pm$ 0.6 
& 65.9 $\pm$ 0.8  \\
TransGAN DeliGAN simp. 10 & & & & & 14.7 & 63.4 % & 61.0
& 52.1 & 66.2 \\ 
TransGAN DeliGAN simp. 100 & & & & & \\ 
TransGAN + 80\% JBT & & & & \\
TransGAN + 90\% JBT & & & & & 15.1 $\pm$ 0.2 
& 64.8 $\pm$ 1.0 
%62.9 $\pm$ 1.3 
& 53.6 $\pm$ 2.4 
& 66.2 $\pm$ 1.4 \\
 \hline
TransGAN, 0.135,0.135 & & & & & 15.3 $\pm$ 0.1  & 63.4 $\pm$ 0.6  & 51.9 $\pm$ 1.1  & 64.2 $\pm$ 0.6 \\ 
0.135,0.138 & & & & & 15.4 $\pm$ 0.1 & 63.4 $\pm$ 1.1  & 53.2 $\pm$ 1.8  & 65.1 $\pm$ 1.3 \\
0.135,0.14 & & & & & 15.4 $\pm$ 0.1  & 63.0 $\pm$ 0.1  & 50.5 $\pm$ 1.4  & 64.0 $\pm$ 1.0 \\
0.135,0.142 & & & & & 15.5 $\pm$ 0.1  & 63.3 $\pm$ 0.9  & 52.2 $\pm$ 1.1 & 63.9 $\pm$ 1.0 \\ \hline
s10, p50, 0.13,0.13 & & & & & 15.5 $\pm$ 0.1 
& 64.5 $\pm$ 0.7 
%61.1 $\pm$ 0.5 
& 53.9 $\pm$ 0.9 
& 65.6 $\pm$ 0.9 \\
0.13,0.14 & & & & & 15.4 $\pm$ 0.1 
& 65.3 $\pm$ 0.7 
%61.4 $\pm$ 1.2 
& 54.8 $\pm$ 1.8 
& 65.5 $\pm$ 1.0 \\\hline
n=30, 0.045,0.045 & & & & & 15.1 $\pm$ 0.1 
& 65.1 $\pm$ 0.6 
%62.3 $\pm$ 0.5 
& 55.6 $\pm$ 0.6 
& 67.1 $\pm$ 0.5 \\ 
0.045,0.048 & & & & & \\
0.045, 0.05 & & & & & 15.1 $\pm$ 0.1 
& 64.8 $\pm$ 0.2 
%61.1 $\pm$ 0.5 
& 55.3 $\pm$ 1.3 
& 66.8 $\pm$ 1.1 \\
0.45,0.505 & & & & & 15.1 $\pm$ 0.1 
& 65.6 $\pm$ 1.3 
%61.5 $\pm$ 0.8 
& 56.3 $\pm$ 1.5 
& 66.4 $\pm$ 1.4 \\ \hline \hline
STL-32 & \\
TransGAN  & & & & & 10.5 $\pm$ 0.1 & 75.7 $\pm$ 0.1 & 87.5 $\pm$ 1.9 & 83.0 $\pm$ 0.2 \\ \hline
TransGAN DeliGAN 10 & & & & & 12.1 $\pm$ 0.1 
& 74.2 $\pm$ 1.2 
%60.2 $\pm$ 0.5 
& 81.5 $\pm$ 1.5 
& 79.6 $\pm$ 0.8 \\
TransGAN DeliGAN 100 & & & & &  \\
TransGAN DeliGAN simp. 10 & & & & & 11.3 $\pm$ 0.1 
& 75.9 $\pm$ 0.8 
%& 59.0 $\pm$ 0.6 
& 85.4 $\pm$ 1.3 
& 82.1 $\pm$ 0.7 \\
TransGAN DeliGAN simp. 100 & & & & & \\ \hline
TransGAN JBT 80\% & & & & & 10.9 $\pm$ 0.1 
& 78.1 $\pm$ 0.3 
%57.6 $\pm$ 1.3 
& 100.3 $\pm$ 2.8 
& 83.8 $\pm$ 0.7 \\  
TransGAN JBT 90\% & & & & & 10.5 $\pm$ 0.0 
& 76.9 $\pm$ 0.1 
%58.8 $\pm$ 0.5 
& 91.9 $\pm$ 1.9 
& 82.1 $\pm$ 0.8 \\ \hline 
TransGAN s5 p20 (0.24,0.24) & & & & & 10.4 $\pm$ 0.1 
& 75.8 $\pm$ 0.8 
%61.3 $\pm$ 0.3 
& 85.3 $\pm$ 2.0 
& 80.8 $\pm$ 1.1 \\ 
(0.24,0.25) & & & & & 10.3 $\pm$ 0.1 
& 75.8 $\pm$ 0.5 
%61.3 $\pm$ 0.5 
& 86.5 $\pm$ 0.6 
& 81.2 $\pm$ 0.9  \\ \hline 
TransGAN s10 p60 (0.135,0.135) & & & & & 10.4 $\pm$ 0.1 & 75.0 $\pm$ 0.5 %& 61.3 $\pm$ 0.7 
& 84.7 $\pm$ 1.4 & 81.1 $\pm$ 0.5 \\
  (0.135,0.138) & \\
  (0.135,0.140) & & & & & 10.4 $\pm$ 0.1 & 74.9 $\pm$ 0.4 %61.6 $\pm$ 1.4 
& 85.8 $\pm$ 1.5 & 82.5 $\pm$ 0.8 \\
  (0.135,0.142) & \\
(0.135,0.144) & & & & & 10.5 $\pm$ 0.1 & 75.0 $\pm$ 0.7 %61.1 $\pm$ 1.0 
& 86.2 $\pm$ 1.4 & 82.2 $\pm$ 0.5 \\ \hline 
TransGAN s10 (0.135,0.135) & & & & & 10.8 $\pm$ 0.1 
& 74.7 $\pm$ 0.3 
%60.6 $\pm$ 1.0 
& 81.6 $\pm$ 1.5 
& 81.3 $\pm$ 1.1 \\
(0.135,0.144) & & & & & 10.8 $\pm$ 0.1 
& 74.7 $\pm$ 0.4 
%& 60.6 $\pm$ 0.5 
& 79.4 $\pm$ 0.9 
& 79.8 $\pm$ 0.7 \\ \hline
TransGAN s100 p20 (0.08,0.08) & & & & & 10.1 $\pm$ 0.1 
& 76.5 $\pm$ 0.9 
%60.2 $\pm$ 0.8 
& 90.0 $\pm$ 3.0 
& 83.0 $\pm$ 0.5 \\ 
(0.08,0.12) & & & & & 9.9 $\pm$ 0.1 
& 76.6 $\pm$ 0.7 
%60.5 $\pm$ 0.7 
& 90.9 $\pm$ 1.3 
& 83.1 $\pm$ 0.8 \\ 
(0.08,0.15) & & & & & 10.0 $\pm$ 0.0 
& 76.9 $\pm$ 0.8 
%59.9 $\pm$ 0.6 
& 91.4 $\pm$ 1.1 
& 83.8 $\pm$ 0.3 \\
(0.08,0.18) & & & & & 10.0 $\pm$ 0.1 
& 77.5 $\pm$ 0.5 
%59.8 $\pm$ 0.8 
& 90.8 $\pm$ 0.8 
& 83.7 $\pm$ 0.6 \\ 
(0.08,0.20) & & & & & 10.0 $\pm$ 0.1 
& 77.8 $\pm$ 0.6 
%59.8 $\pm$ 0.8 
& 94.1 $\pm$ 0.9 
& 83.5 $\pm$ 0.8 \\\hline
TransGAN s10 p200 (0.13,0.13) & & & & & 12.1 & 73.0 %&61.1 
& 78.1 & 77.3 \\

\end{tabular}
\end{table*}


\begin{table*}[h]
\small
\centering
\begin{tabular}{l|c|c|c|c|c|c|c} 
Dataset & Width &  LogReg & Convex & FD & Prec. & Dens. & Cov. \\ 
& & Acc. & Acc. & & & \\\hline
CIFAR- & 32 & 53.4 $\pm$ 0.5 & 61.1 $\pm$ 0.3 & 447.9 $\pm$ 15.6  & 63.8 $\pm$ 0.7  & 52.9 $\pm$ 1.3 & 73.0 $\pm$ 1.0   \\
10 & 64 & 60.7 $\pm$ 0.5 & 72.1 $\pm$ 0.6 & 154.3 $\pm$ 10.8  & 72.1 $\pm$ 0.4  &  69.4 $\pm$ 1.5 & 82.9 $\pm$ 0.7 \\
(ResNet) & 128 & 63.4 $\pm$ 0.4  & 73.1 $\pm$ 0.6 & 94.5 $\pm$ 11.4  & 74.9 $\pm$ 1.0  &  74.2 $\pm$ 2.3 & 85.7 $\pm$ 1.0 \\ 
& 256 & {65.0} $\pm$ 0.4 & \textbf{75.4} $\pm$ 0.4 & 75.8 $\pm$ 8.6  &75.6 $\pm$ 0.4  &  76.9 $\pm$ 1.3 & \textbf{87.5 $\pm$ 0.8} \\ 
& 512 & \textbf{65.3} $\pm$ 0.6 & 75.2 $\pm$ 0.7  &  \textbf{ 70.8} $\pm$ 6.0 & \textbf{76.6} $\pm$ 1.0  & \textbf{77.5} $\pm$ 2.2 & 87.0 $\pm$ 0.6 \\ \hline
CIFAR- & 32 & 20.3 $\pm$ 0.1 & 28.1 $\pm$ 0.5 &  462.3 $\pm$ 15.1  & 49.3 $\pm$ 0.6  &  37.9 $\pm$ 1.6 & 69.5 $\pm$ 1.6 \\
100 & 64 & 23.7 $\pm$ 0.9 &  33.4 $\pm$ 0.5 &  286.4 $\pm$ 10.4  & 58.7 $\pm$ 0.7  &  49.4 $\pm$ 1.4 & 78.7 $\pm$ 1.6 \\
(ResNet)  & 128 & 28.4 $\pm$ 0.3 & 39.1 $\pm$ 0.7 & 139.1 $\pm$ 11.8 & 65.6 $\pm$ 0.7 &  64.3 $\pm$ 2.3 & 85.9 $\pm$ 0.7 \\
& 256 & 32.2 $\pm$ 0.5 & 45.1 $\pm$ 0.6 &  117.4 $\pm$ 8.2 & \textbf{66.0} $\pm$ 0.9 & \textbf{64.6} $\pm$ 1.8 & \textbf{86.4} $\pm$ 0.5  \\
& 512 & \textbf{34.4} $\pm$ 0.5 & \textbf{47.1} $\pm$ 0.5 &  \textbf{115.3} $\pm$ 9.0 & 65.9 $\pm$ 0.5 & 64.3 $\pm$ 1.4 & 85.9 $\pm$ 0.5 \\
\end{tabular}
\caption{\textit{Overparametrization study (dataset-specific classifier)}: 
for a latent dimension equal to $64$, we vary the width of the generator (confidence intervals computed on 10 checkpoints). Increasing the capacity of GANs tend to structure their latent space in simplicial clusters (better LogReg accuracy) and improve their performance on precision, density and coverage. \label{table:overparametrization_study}}
\end{table*}

\begin{table}[H]
\begin{tabular}{l|c|c|c|c|c|c|c}
Dataset & L. Dim.  & Acc. & FD & Prec. & Rec. & Dens. & Cov. \\ \hline 
MNIST & 2 & 44.3 $\pm$ 2.5 & 112.3 $\pm$ 22.6 & 2.9 $\pm$ 1.0 & 89.1 $\pm$ 2.0 & 0.9 $\pm$ 0.3 & 2.1 $\pm$ 0.5 \\ 
& 4 & 59.4 $\pm$ 0.7 & 36.4 $\pm$ 9.3 & 75.7 $\pm$ 1.8 & 91.5 $\pm$ 0.5 & 47.9 $\pm$ 2.2 & 66.0 $\pm$ 2.0 \\
& 6 & 83.9 $\pm$ 0.4 & 15.4 $\pm$ 3.0 & 90.0 $\pm$ 0.7 & 92.4 $\pm$ 0.7 & 76.3 $\pm$ 2.0 & 85.8 $\pm$ 0.4 \\
& 8 & 84.7 $\pm$ 0.4 & 18.2 $\pm$ 3.4 & 91.1 $\pm$ 0.7 & 92.3 $\pm$ 0.5 & 81.3 $\pm$ 2.2 & 87.1 $\pm$ 0.8 \\ 
& 10 & 86.7 $\pm$ 0.4 & 10.7 $\pm$ 2.6 & 93.3 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 89.0 $\pm$ 2.2 & 89.8 $\pm$ 0.7 \\
  & 12 & 87.4 $\pm$ 0.4 & 7.2 $\pm$ 1.6 & 94.6 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 94.3 $\pm$ 2.0 & 91.8 $\pm$ 0.7 \\
  & 16 & 86.9 $\pm$ 0.4 & 11.0 $\pm$ 1.0 & 93.8 $\pm$ 0.3 & 91.8 $\pm$ 0.6 & 92.2 $\pm$ 0.9 & 90.7 $\pm$ 0.5 \\
  & 32 & 90.3 $\pm$ 0.4 & 10.4 $\pm$ 1.6 & 93.6 $\pm$ 0.3 & 91.6 $\pm$ 0.7 & 91.8 $\pm$ 1.7 & 90.3 $\pm$ 0.6 \\
  & 64 & 90.4 $\pm$ 0.3 & 13.3 $\pm$ 2.6 & 93.2 $\pm$ 0.4 & 92.3 $\pm$ 0.5 & 90.1 $\pm$ 2.0 & 90.2 $\pm$ 0.8 \\
  & 128 & 87.0 $\pm$ 0.4 &  11.0 $\pm$ 2.3 & 93.6 $\pm$ 0.3 & 91.8 $\pm$ 0.4 & 91.6 $\pm$ 1.5 & 90.4 $\pm$ 0.7 \\ \hline 
 CIFAR-10 & 2 & 22.7 $\pm$ 1.7 & 450.5 $\pm$ 25.6  & 5.9 $\pm$ 0.7  & 83.9 $\pm$ 1.0  & 1.8 $\pm$ 0.2  & 4.1 $\pm$ 0.4 \\
 & 5 & 35.3 $\pm$ 0.5 & 183.1 $\pm$ 10.7  & 64.0 $\pm$ 0.6  & 82.6 $\pm$ 0.6  & 51.8 $\pm$ 1.0  & 74.8 $\pm$ 0.7 \\ 
 & 10 & 52.5 $\pm$ 0.3  & 117.6 $\pm$ 7.2  & 71.2 $\pm$ 0.4  & 82.3 $\pm$ 0.5  & 65.6 $\pm$ 1.1  & 82.3 $\pm$ 0.7 \\
 & 30 & 64.2 $\pm$ 0.5 & 89.8 $\pm$ 7.0  & 75.1 $\pm$ 0.7  & 81.4 $\pm$ 0.8  & 76.0 $\pm$ 1.8  & 85.9 $\pm$ 0.8  \\ 
 & 128 & 64.1 $\pm$ 0.5 & 81.3 $\pm$ 10.7  & 75.6 $\pm$ 0.5  & 81.8 $\pm$ 0.5  & 76.2 $\pm$ 1.6  & 86.7 $\pm$ 0.6 \\ \hline
 Synthetic & 2 & 25.0 $\pm$ 3.0 & 175.9 $\pm$ 19.6  & 7.9 $\pm$ 0.8  & 78.3 $\pm$ 1.2  & 2.4 $\pm$ 0.3  & 5.1 $\pm$ 0.7 \\
 CIFAR-10 & 5 & 35.3 $\pm$ 0.5 & 183.1 $\pm$ 10.7  & 64.0 $\pm$ 0.6  & 82.6 $\pm$ 0.6 & 51.8 $\pm$ 1.0  & 74.8 $\pm$ 0.7 \\
 & 10 & 48.3 $\pm$ 0.6 & 131.7 $\pm$ 28.5  & 58.8 $\pm$ 4.0  & 78.2 $\pm$ 1.0  & 59.0 $\pm$ 6.2  & 74.6 $\pm$ 3.7 \\
 & 30 & 57.3 $\pm$ 0.9 & 57.7 $\pm$ 11.1  & 73.6 $\pm$ 2.0  & 76.7 $\pm$ 0.8  & 79.3 $\pm$ 5.4  & 90.4 $\pm$ 1.3  \\ 
 & 128 & 55.7 $\pm$ 1.0  & 79.0 $\pm$ 12.4  & 71.3 $\pm$ 2.9  & 77.7 $\pm$ 1.6  & 71.4 $\pm$ 8.1  & 84.2 $\pm$ 6.3 \\ \hline
 CIFAR-100 & 2 & 12.1 $\pm$ 1.2 & 912.4 $\pm$ 125.8  & 1.7 $\pm$ 0.3  & 86.2 $\pm$ 0.9  & 0.5 $\pm$ 0.1  & 0.9 $\pm$ 0.1  \\
 & 5 & 11.1 $\pm$ 0.3 & 244.9 $\pm$ 8.7  & 49.5 $\pm$ 0.8  & 81.9 $\pm$ 0.3  & 34.9 $\pm$ 0.9  & 64.4 $\pm$ 1.2 \\
 & 10 & 21.7 $\pm$ 0.3  & 220.2 $\pm$ 10.2  & 57.7 $\pm$ 0.7  & 81.6 $\pm$ 0.7  & 47.7 $\pm$ 1.3  & 76.9 $\pm$ 1.0 \\
 & 30 & 27.3 $\pm$ 0.4 & 198.7 $\pm$ 14.8  & 61.2 $\pm$ 0.6  & 80.7 $\pm$ 0.6  & 54.6 $\pm$ 1.4  & 81.7 $\pm$ 0.9 \\
 & 64 & 28.4 $\pm$ 0.3 & 139.1 $\pm$ 11.8 & 65.6 $\pm$ 0.7 & 79.5 $\pm$ 0.6 & 64.3 $\pm$ 2.3 & 85.9 $\pm$ 0.7 \\
 & 128 & 26.7 $\pm$ 0.5  &  191.9 $\pm$ 10.7 & 61.7 $\pm$ 0.8  & 80.2 $\pm$ 0.8  & 56.4 $\pm$ 1.2  & 82.5 $\pm$ 1.0  \\
%Synthetic Mnist & 2 & 34.4 $\pm$ 5.3  & 53.8 $\pm$ 5.8 & 0.5 $\pm$ 0.4 & 59.6 $\pm$ 3.9 & 0.1 $\pm$ 0.1 & 0.2 $\pm$ 0.1\\ 
%& 8 & 72.5 $\pm$ 1.5 & 17.8 $\pm$ 1.4 & 86.2 $\pm$ 1.2 & 57.8 $\pm$ 3.2 & 64.3 $\pm$ 3.1 & 50.6 $\pm$ 1.8  \\
%& 16 & 73.5 $\pm$ 0.8 & 20.4 $\pm$ 1.1 & 88.2 $\pm$ 1.1 & 56.7 $\pm$ 1.8 & 69.5 $\pm$ 1.6 & 49.1 $\pm$ 2.0 \\
%& & \\\hline
\end{tabular}
\caption{Performance of GANs when varying latent space dimension. Confidence intervals are computed on 10 checkpoints of the same training. See main paper for curves of precision and FID with regard to the latent space dimension.\label{appendix:full_results_v2} }
\end{table}


\begin{table}[H]
\begin{tabular}{l|c|c|c|c|c|c|c}
Dataset & L. Dim.  & Acc. & FD & Prec. & Rec. & Dens. & Cov. \\ \hline 
MNIST & 2 & 44.3 $\pm$ 2.5 & 112.3 $\pm$ 22.6 & 2.9 $\pm$ 1.0 & 89.1 $\pm$ 2.0 & 0.9 $\pm$ 0.3 & 2.1 $\pm$ 0.5 \\ 
& 4 & 59.4 $\pm$ 0.7 & 36.4 $\pm$ 9.3 & 75.7 $\pm$ 1.8 & 91.5 $\pm$ 0.5 & 47.9 $\pm$ 2.2 & 66.0 $\pm$ 2.0 \\
& 6 & 83.9 $\pm$ 0.4 & 15.4 $\pm$ 3.0 & 90.0 $\pm$ 0.7 & 92.4 $\pm$ 0.7 & 76.3 $\pm$ 2.0 & 85.8 $\pm$ 0.4 \\
& 8 & 84.7 $\pm$ 0.4 & 18.2 $\pm$ 3.4 & 91.1 $\pm$ 0.7 & 92.3 $\pm$ 0.5 & 81.3 $\pm$ 2.2 & 87.1 $\pm$ 0.8 \\ 
& 10 & 86.7 $\pm$ 0.4 & 10.7 $\pm$ 2.6 & 93.3 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 89.0 $\pm$ 2.2 & 89.8 $\pm$ 0.7 \\
  & 12 & 87.4 $\pm$ 0.4 & 7.2 $\pm$ 1.6 & 94.6 $\pm$ 0.5 & 91.5 $\pm$ 0.5 & 94.3 $\pm$ 2.0 & 91.8 $\pm$ 0.7 \\
  & 16 & 86.9 $\pm$ 0.4 & 11.0 $\pm$ 1.0 & 93.8 $\pm$ 0.3 & 91.8 $\pm$ 0.6 & 92.2 $\pm$ 0.9 & 90.7 $\pm$ 0.5 \\
  & 32 & 90.3 $\pm$ 0.4 & 10.4 $\pm$ 1.6 & 93.6 $\pm$ 0.3 & 91.6 $\pm$ 0.7 & 91.8 $\pm$ 1.7 & 90.3 $\pm$ 0.6 \\
  & 64 & 90.4 $\pm$ 0.3 & 13.3 $\pm$ 2.6 & 93.2 $\pm$ 0.4 & 92.3 $\pm$ 0.5 & 90.1 $\pm$ 2.0 & 90.2 $\pm$ 0.8 \\
  & 128 & 87.0 $\pm$ 0.4 &  11.0 $\pm$ 2.3 & 93.6 $\pm$ 0.3 & 91.8 $\pm$ 0.4 & 91.6 $\pm$ 1.5 & 90.4 $\pm$ 0.7 \\ \hline 
 CIFAR-10 & 2 & 22.7 $\pm$ 1.7 & 44.2 $\pm$ 1.0 & 4.2 $\pm$ 0.9 & 61.3 $\pm$ 0.7 & 1.2 $\pm$ 0.3 & 1.5 $\pm$ 0.4 \\ 
 & 5 & 35.3 $\pm$ 0.5 & 22.7 $\pm$ 0.4 & 57.6 $\pm$ 0.7 & 63.2 $\pm$ 0.7 & 49.8 $\pm$ 1.2 & 57.1 $\pm$ 1.0\\ 
 & 10 & 52.5 $\pm$ 0.3 & 20.2 $\pm$ 0.2 & 62.6 $\pm$ 0.6 & 64.7 $\pm$ 0.6 & 61.2 $\pm$ 1.3 & 67.1 $\pm$ 0.7  \\
 & 15 &  57.8 $\pm$ 0.3 & 18.7 $\pm$ 0.5 & 65.3 $\pm$ 0.3 & 64.6 $\pm$ 0.5 & 69.3 $\pm$ 1.0 & 72.6 $\pm$ 0.9 \\
 & 30 & 64.2 $\pm$ 0.5 & 17.4 $\pm$ 0.3 & 66.4 $\pm$ 0.4 & 64.5 $\pm$ 0.8 & 72.0 $\pm$ 1.8 & 74.9 $\pm$ 0.7 \\ 
 & 64 &  63.9 $\pm$ 0.4 & 17.0 $\pm$ 0.3 & 65.7 $\pm$ 0.5 & 64.7 $\pm$ 0.5 & 70.6 $\pm$ 1.5 & 75.2 $\pm$ 0.7 \\
 & 128 & 64.1 $\pm$ 0.5 & 16.7 $\pm$ 0.4 & 66.5 $\pm$ 0.6 & 64.5 $\pm$ 0.6 & 73.6 $\pm$ 1.9 & 76.1 $\pm$ 0.9  \\ \hline
 Synthetic & 2 & 25.0 $\pm$ 3.0 & 24.5 $\pm$ 2.0 
& 4.3 $\pm$ 0.7 
& 65.2 $\pm$ 0.9 
& 1.1 $\pm$ 0.2 
& 2.2 $\pm$ 0.4   \\
 CIFAR-10 & 5 & 35.3 $\pm$ 0.5 &  6.7 $\pm$ 0.3 
& 58.0 $\pm$ 0.8 
& 73.8 $\pm$ 0.5 
& 50.3 $\pm$ 1.7 
& 74.2 $\pm$ 1.1 \\
 & 10 & 48.3 $\pm$ 0.6 & 8.2 $\pm$ 0.9 
& 63.7 $\pm$ 3.4 
& 74.2 $\pm$ 1.7 
& 57.8 $\pm$ 3.4 
& 74.6 $\pm$ 3.9 \\
 & 30 & 57.3 $\pm$ 0.9 &  6.2 $\pm$ 0.3 
& 68.0 $\pm$ 3.8 
& 72.5 $\pm$ 1.0 
& 74.6 $\pm$ 2.4 
& 76.3 $\pm$ 1.7  \\ 
 & 128 & 55.7 $\pm$ 1.0 & 7.2 $\pm$ 1.9 
& 67.2 $\pm$ 4.0 
& 73.9 $\pm$ 1.3 
& 72.3 $\pm$ 4.8 
& 75.4 $\pm$ 5.7\\ \hline
 CIFAR-100 & 2 & 12.1 $\pm$ 1.2 & 49.8 $\pm$ 3.2 & 4.2 $\pm$ 0.7 & 63.7 $\pm$ 1.3 & 1.1 $\pm$ 0.2 & 1.3 $\pm$ 0.2 \\
 & 5 & 11.1 $\pm$ 0.3  & 23.6 $\pm$ 0.2 & 52.2 $\pm$ 0.7 & 65.1 $\pm$ 0.8 & 40.0 $\pm$ 1.1 & 52.3 $\pm$ 0.9\\
 & 10 & 21.7 $\pm$ 0.3 & 22.2 $\pm$ 0.3 & 58.1 $\pm$ 0.4 & 65.3 $\pm$ 0.6 & 52.9 $\pm$ 0.9 & 63.5 $\pm$ 0.9   \\
 & 30 & 27.3 $\pm$ 0.4  & 21.4 $\pm$ 0.2 & 60.5 $\pm$ 0.4 & 65.2 $\pm$ 0.7 & 59.3 $\pm$ 0.9 & 67.9 $\pm$ 0.9  \\
 & 64 & 28.4 $\pm$ 0.3 & 21.2 $\pm$ 0.3 & 61.2 $\pm$ 0.3 & 63.8 $\pm$ 0.8 & 60.1 $\pm$ 0.7 & 69.5 $\pm$ 0.8 \\
 & 128 & 26.7 $\pm$ 0.5 & 21.6 $\pm$ 0.2 & 60.5 $\pm$ 0.4 & 64.4 $\pm$ 0.9 & 59.8 $\pm$ 0.8 & 69.3 $\pm$ 0.8 \\
%Synthetic Mnist & 2 & 34.4 $\pm$ 5.3  & 53.8 $\pm$ 5.8 & 0.5 $\pm$ 0.4 & 59.6 $\pm$ 3.9 & 0.1 $\pm$ 0.1 & 0.2 $\pm$ 0.1\\ 
%& 8 & 72.5 $\pm$ 1.5 & 17.8 $\pm$ 1.4 & 86.2 $\pm$ 1.2 & 57.8 $\pm$ 3.2 & 64.3 $\pm$ 3.1 & 50.6 $\pm$ 1.8  \\
%& 16 & 73.5 $\pm$ 0.8 & 20.4 $\pm$ 1.1 & 88.2 $\pm$ 1.1 & 56.7 $\pm$ 1.8 & 69.5 $\pm$ 1.6 & 49.1 $\pm$ 2.0 \\
%& & \\\hline
\end{tabular}
\caption{ Performance of GANs when varying latent space dimension. Confidence intervals are computed on 10 checkpoints of the same training. See main paper for curves of precision and FID with regard to the latent space dimension. On MNIST, a MNIST classifier is used. On CIFAR datasets, Inception Net is used. \label{appendix:full_results_v3} }
\end{table}
